Semi-supervised Classification using Attention-based Regularization on Coarse-resolution Data

Many real-world phenomena are observed at multiple resolutions. Predictive models designed to predict these phenomena typically consider different resolutions separately. This approach might be limiting in applications where predictions are desired at fine resolutions but available training data is scarce. In this paper, we propose classification algorithms that leverage supervision from coarser resolutions to help train models on finer resolutions. The different resolutions are modeled as different views of the data in a multi-view framework that exploits the complementarity of features across different views to improve models on both views. Unlike traditional multi-view learning problems, the key challenge in our case is that there is no one-to-one correspondence between instances across different views in our case, which requires explicit modeling of the correspondence of instances across resolutions. We propose to use the features of instances at different resolutions to learn the correspondence between instances across resolutions using an attention mechanism.Experiments on the real-world application of mapping urban areas using satellite observations and sentiment classification on text data show the effectiveness of the proposed methods.

==> bibfile.tex <==
\begin{thebibliography}{99} 

\bibitem{AtluriSurvey} Atluri, Gowtham, Anuj Karpatne, and Vipin Kumar. "Spatio-temporal data mining: A survey of problems and methods." ACM Computing Surveys (CSUR) 51.4 (2018): 83.

\bibitem{AnujMagazine} Karpatne, Anuj, et al. "Monitoring land-cover changes: A machine-learning perspective." IEEE Geoscience and Remote Sensing Magazine 4.2 (2016): 8-21.

\bibitem{UNreport} United Nations, Department of Economic and Social Affairs, Population Division (2014).
World Urbanization Prospects: The 2014 Revision, Highlights (ST/ESA/SER.A/352).

\bibitem{Urban1} Li X, Gong P. Urban growth models: progress and perspective. Science bulletin. 2016 Nov 1;61(21):1637-50.

\bibitem{Urban2} Ranger N, Hallegatte S, Bhattacharya S, Bachu M, Priya S, Dhore K, Rafique F, Mathur P, Naville N, Henriet F, Herweijer C. An assessment of the potential impact of climate change on flood risk in Mumbai. Climatic change. 2011 Jan 1;104(1):139-67.

\bibitem{UrbanNews} https://www.theguardian.com/cities/2014/nov/24/mumbai-verge-imploding-polluted-megacity

\bibitem{MILSurvey1} Foulds, James, and Eibe Frank. "A review of multi-instance learning assumptions." The Knowledge Engineering Review 25.1 (2010): 1-25.

\bibitem{MILSurvey2} Cheplygina, Veronika, David MJ Tax, and Marco Loog. "On classification with bags, groups and sets." Pattern recognition letters 59 (2015): 11-17.

\bibitem{MILR} Ray, Soumya, and Mark Craven. "Supervised versus multiple instance learning: An empirical comparison." Proceedings of the 22nd international conference on Machine learning. ACM, 2005.


\bibitem{AttentionNLP} Galassi, Andrea, Marco Lippi, and Paolo Torroni. "Attention, please! A Critical Review of Neural Attention Models in Natural Language Processing." arXiv preprint arXiv:1902.02181 (2019).

\bibitem{zhouWLIntro} Zhou, Zhi-Hua. "A brief introduction to weakly supervised learning." National Science Review 5.1 (2017): 44-53.


\end{thebibliography}

==> conclusion.tex <==
\section{Conclusion}
In this paper, we formalized the problem of classifying spatio-temporal phenomena simultaneously at multiple resolutions in a multi-view framework. The multi-view framework helps to regularize the models trained on individual resolutions by enforcing consistency of predictions across resolutions on the large number of freely-available unlabeled data. Unlike traditional multi-view learning scenarios, the multi-resolution classification task involves a many-to-one correspondence between views of the data, which the proposed methods in the paper learn explicitly through multiple instance learning and attention mechanism. Experiments on urban mapping data sets show the utility of utilizing unlabeled data through the multi-view framework. %Future work involves investigating other approaches to modeling the consistency across resolutions such as through the attention mechanism \cite{AttentionNLP} that has shown much promise in domains such as Natural Language Processing (NLP).

==> evaluation.tex <==
\section{Evaluation} \label{evaluationSection}

\begin{table*}[t]
    \centering
    \caption{Comparison with baselines: balanced data sets (Accuracy)}
    \begin{tabular}{|*{5}{c|}}
    \hline 
    \multicolumn{2}{|c|}{\multirow{2}{*}{METHODS}} & \multicolumn{3}{c|}{DATASETS}\\\cline{3-5}
    \multicolumn{2}{|c|}{\multirow{2}{*}{}} & MINNEAPOLIS & MADRID & ROME\\\hline
    \multirow{4}{*}{LANDSAT} & LogReg & 0.8842 & 0.9405 & 0.905\\\cline{2-5}
    & Conc Features & 0.8983 & 0.9437 & 0.914\\\cline{2-5}
    & Semi Supervised & 0.8877 & 0.943 & 0.9085\\\cline{2-5}
    & Multi-Res & 0.9231 & 0.9644 & 0.9591\\\hline
    \multirow{4}{*}{SENTINEL} & LogReg & 0.9335 & 0.9218 & 0.9321\\\cline{2-5}
    & Conc Features & 0.9458 & 0.9392 & 0.9384\\\cline{2-5}
    & Semi Supervised & 0.9443 & 0.9364 & 0.9328\\\cline{2-5}
    & Multi-Res & 0.9571 & 0.9434 & 0.9469\\\hline
    \end{tabular}
    \label{tab:result}
\end{table*}

\subsection{Background and motivation: Why study urbanization?}
The World Urbanization Prospects report \cite{UNreport} estimates that about 2.29 billion people live in urban areas accounting for 54\% of the world’s human population. As the world’s population goes up, increasing number of people migrate to urban areas in search of better quality of living. It is projected that the urban population will increase by another 2.5 billion by the year 2050 and about 2.25 billion of this urban growth will occur in developing regions of Asia and Africa. As the Director of the United Nations Population Division said, managing urban areas has become one of the most important developmental challenges of the 21st century. Urbanization is beneficial from a sustainability standpoint since it is resourcefully more economical and environmentally less damaging to provide for a concentrated population than a dispersed one \cite{UNreport}. However, rapid unchecked urbanization can have adverse environmental and ecological issues \cite{Urban1, Urban2} along with poor living conditions \cite{UrbanNews}. Thus, an urban planning agenda is critical to ensure our sustainable living on the planet. This requires that we have regularly updated maps for urban land and population density to track their dynamics.

\begin{figure}
\centering
\includegraphics[width = \linewidth]{IMAGES/UNreportGraphic.png}
\caption{Most urban expansion is occurring in developing nations where deploying resource-intensive methods is not an option. Figure courtesy of \cite{UNreport}.}%
\label{fig:UNgraphic}%
\end{figure}

\begin{table*}[t]
    \begin{center}
        \caption{Dataset details}
        \label{tab:result}
        \begin{tabular}{|c|c|p{1.7cm}|c|p{1cm}|c|p{1.7cm}|c|p{1cm}|}
            \hline
            \multirow{2}{*}{REGION} & \multicolumn{4}{c|}{LANDSAT} & \multicolumn{4}{c|}{SENTINEL}\\\cline{2-9}
            & TILE SIZE & LABELED \newline TRAIN & UNLABELED & TEST & TILE SIZE & LABELED TRAIN & UNLABELED & TEST\\\hline
            MINNEAPOLIS & 3660$\times$3660 & 1000 & 10000 & 60000 & 10980$\times$10980 & 1000 & 90000 & 60000\\\hline
            MADRID & 3660$\times$3660 & 1000 & 10000 & 60000 & 10980$\times$10980 & 1000 & 90000 & 60000\\\hline
            ROME & 3660$\times$3660 & 1000 & 10000 & 60000 & 10980$\times$10980 & 1000 & 90000 & 60000\\\hline
        \end{tabular}
    \end{center}
\end{table*}

The methods proposed in this paper are evaluated on data-sets of 3 different regions from a real world application - urban area detection, that use satellite-collected observations of different locations to automatically track changes changes on the surface of the Earth. We use data-sets from two satellites available at two different resolutions. Landsat 8 satellite data product having 30m spatial resolution and Sentinel 2A data product having 10m spatial resolution. These two sources act as the coarse and fine resolution respectively. We use the three tiles from each source each of which surround the region of Minneapolis, Madrid and Rome. In our experiments we evaluate the performance of the following methods on the data-sets in table~\ref{tab:data-sets}.
\begin{itemize}
    \item \textbf{Coarse-Resolution Logistic Regression and Fine-resolution Logistic Regression} In this method, we only use the coarse-resolution and the fine-resolution data to learn two separate models and evaluate their performance.
    \item \textbf{Concatenated Features Logistic Regression} In this method we learn two models, one at coarse-resolution and the other at fine-resolution. In case of the first model for each coarse-resolution pixel, the corresponding fine-resolution pixels are averaged and concatenated to have an extended feature-set. The same is done for each fine-resolution pixel in the second model. Thus we have an extended features coarse-resolution data-set and an extended features fine-resolution data-set on which two separate models are learned. 
    \item \textbf{Semi-Supervised Logistic Regression} This method makes uses of the large number of the unlabeled data along with the labeled data to learn two separate models at both resolutions.
    \item \textbf{Multi-Resolution Logistic Regression} Proposed algorithm which uses the limited labeled data available in the respective resolutions as well as enforcing consistency in predictions over the large number of unlabeled data available in both resolutions for the same region. 
\end{itemize}

\subsection{Discussion}
We evaluate the performance on the balanced data sets using accuracy as shown in table~\ref{tab:result}. As expected, logistic regression performs the worst since it is limited to the small labeled data as well as single feature set. Although concatenated features logistic regression is a step ahead as it uses two independent feature sets one available from the coarse-resolution and the other available from the fine-resolution data-set, it does not make use of the unlabeled data. Similarly, semi-supervised logistic regression uses the unlabeled data resulting in a slight increase in performance but it is limited to a single feature-set. Our multi-view approach has the advantage of using the independent feature sets providing richer information as well as the two models are tied by a consistency loss which helps in learning form each other. 


\begin{table}
    \centering
    \caption{Comparison with baselines: balanced data-sets (Accuracy)}
    % \hskip-1.6cm
    \begin{tabular}{|*{4}{c|}}
    \hline 
    \multicolumn{2}{|c|}{\multirow{2}{*}{METHODS}} & \multicolumn{2}{c|}{DATASETS}\\\cline{3-4}
    \multicolumn{2}{|c|}{\multirow{2}{*}{}} & ROME & MINNEAPOLIS\\\hline
    \multirow{4}{*}{LANDSAT} & LogReg & 0.877 & 0.887\\\cline{2-4}
    & Conc Features & 0.822 & 0.821\\\cline{2-4}
    & Semi Supervised & 0.876 & 0.888\\\cline{2-4}
    & Multi-Res & \textbf{0.913} & \textbf{0.917}\\\hline
    \multirow{4}{*}{SENTINEL} & LogReg & 0.852 & 0.884\\\cline{2-4}
    & Conc Features & 0.874 & 0.896\\\cline{2-4}
    & Semi Supervised & 0.884 & 0.899\\\cline{2-4}
    & Multi-Res & \textbf{0.944} & \textbf{0.952}\\\hline
    \end{tabular}
    \label{tab:result}
\end{table}

The methods proposed in this paper are evaluated on data-sets of 2 different regions namely Minneapolis and Rome, from a real world application - urban area detection, that use satellite-collected observations of different locations to automatically track changes on the surface of the Earth. We use data-sets from two satellites available at two different resolutions. Landsat 8 satellite data product having 30m spatial resolution(3660$\times$3660 pixels) and Sentinel 2A data product having 10m spatial resolution(10980$\times$10980 pixels). These two sources act as the coarse and fine resolution respectively. 
%In our experiments we take training samples from one quarter of the image and test it on the rest three quarters. 
In each data-set we take 200 training samples and 60000 test samples on each resolution. In addition to those we also have 10000 unlabeled coarse-resolution and correspondingly, 90000 unlabeled fine-resolution samples (there are 9 Sentinel pixels for each Landsat pixel). We compare the following methods on the above data-sets: \\ \hfill
\textbf{1. Coarse-Resolution Logistic Regression and Fine-resolution Logistic Regression} Separate models are trained on both resolutions using their respective labeled samples. \\ \hfill
\textbf{2. Concatenated Features Logistic Regression} This method uses a concatenated feature space using features from the other resolution. For each coarse-resolution pixel, the corresponding fine-resolution pixels are averaged and concatenated to have an extended feature-set. The same is done for each fine-resolution pixel. Separate models are learned at each resolution using the extended feature sets. \\ \hfill
\textbf{3. Semi-Supervised Logistic Regression} This is an extension of baseline 1 where in addition to labeled samples at a given resolution, unlabeled samples are also used to regularize predictions at that resolution. Note that models at different resolutions are still trained separately.\\ \hfill
\textbf{4. Multi-Resolution Logistic Regression} Proposed algorithm which uses the limited labeled data available in the respective resolutions and enforces consistency in predictions on unlabeled data between resolutions. \vspace{-3mm}

\subsection{Results}
Table~\ref{tab:result} reports the accuracy for the two data sets for the urban mapping application i.e Rome and Minneapolis. First, we have \emph{LogReg}, that is trained with just labeled samples from each resolution. If we concatenate features from the other resolution (\emph{Conc Features}), we observe that the performance goes down since there are not enough samples to handle the increased dimensionality. Using unlabeled data in a semi-supervised fashion yields some benefit, especially in the finer resolution. However, the most gains are found in using unlabeled data to enforce consistency between resolutions as it brings out the benefit of an independent feature space to learn from.

==> evaluation_v1.tex <==
\section{Evaluation} \label{evaluationSection}
We evaluate the methods proposed in this paper on data-sets of 3 different regions from a real world application - urban area detection, that use satellite-collected observations of different locations to automatically track changes changes on the surface of the Earth. We use data-sets from two satellites available at two different resolutions. Landsat 8 satellite data product having 30m spatial resolution and Sentinel 2A data product having 10m spatial resolution. These two sources act as the coarse and fine resolution respectively. We use the three tiles from each source each of which surround the region of Minneapolis, Madrid and Rome. We also perform a case study of our method on sentiment classification of reviews from the Large Movie Review Dataset \cite{imdb}. For sentence level labels we used the labeled sentences for the imdb dataset from \cite{imdbSentence}. Thus the sentence labels are fine resolution labels whereas the reviews being a collection of sentences act as the coarse resolution labels.

\begin{table*}[t]
    \begin{center}
        \caption{Dataset details}
        \label{tab:tableData}
        \begin{tabular}{|c|l|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{Data set} & \multirow{2}{*}{Task} & \multicolumn{2}{c|}{COARSE} & \multicolumn{3}{c|}{FINE}\\\cline{3-7}
            & &TRAIN & UNLABELED & TRAIN & UNLABELED & TEST\\\hline
            D1 & Urban mapping, Minneapolis& 2000 & 10000 & 200 & 90000 & 60000\\\hline
            D2 & Urban mapping, Madrid& 2000 & 10000 & 200 & 90000 & 60000\\\hline
            D3 & Urban mapping, Rome& 2000 & 10000 & 200 & 90000 & 60000\\\hline
            D4 & Sentiment classification, IMDB reviews& 2000 & 1000 & 200 & 10000 & 236\\\hline
        \end{tabular}
    \end{center}
\end{table*}

\subsection{Comparison with baselines}
For our experiments, we compare the performance of our method (called \emph{MultiRes-Attention}) against the following baselines: \hfill \\
\textbf{1. Fine-resolution Logistic Regression} In this method, we only use the fine-resolution data to learn two separate models and evaluate their performance. \hfill \\
\textbf{2. SSRManifold \cite{SSRManifold}} Manifold regularization is a class of semi-supervised techniques where unlabeled instances close to one another in the feature space are expected to have similar predictions. Here, we use the formulation proposed in \cite{SSRManifold} using Euclidean distance and assuming a fully connected graph for computing neighborhood. This method makes uses of the large number of the unlabeled data along with the labeled data to learn two separate models at both resolutions.\hfill \\
\textbf{3. Augment} \cite{augment} In this method, first we only use the coarse-resolution and the fine-resolution data to learn two separate models. This method then greedily increases the labeled set on both resolutions based on instances where the predictions on both resolutions agree\hfill \\
\textbf{4. WeaSL} Train base model on the coarse resolution. Predict the label on all unlabled coarse resolution instances. Then propogate the predicted label to fine resolution. Add this to the pool of fine resolution labels. Train base model on fine resolution with the new labeled set. %\hfill

\begin{table}[h]
  \centering
  \caption{Comparison with baselines: balanced case}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    Method &  D1 & D2 & D3 & D4\\ \hline
    OnlyStrong & $\underset{(0.111)}{0.59}$ & $\underset{(0.059)}{0.68}$ & $\underset{(0.066)}{0.64}$ & $\underset{(0.011)}{0.62}$\\ \hline
    SSRManifold & $\underset{(0.079)}{0.63}$ & $\underset{(0.041)}{0.70}$ & $\underset{(0.049)}{0.69}$ & $\underset{(0.015)}{0.64}$\\ \hline
    WeaSL & $\underset{(0.082)}{0.71}$ & $\underset{(0.044)}{0.81}$ & $\underset{(0.008)}{0.82}$ & $\underset{(0.012)}{0.66}$\\ \hline
    Augment & $\underset{(0.117)}{0.687}$ & $\underset{(0.072)}{0.72}$&  $\underset{(0.042)}{0.73}$ & $\underset{(0.015)}{0.66}$\\ \hline
    \begin{tabular}{@{}c@{}}Multi-Res \\ MIL\end{tabular} & $\underset{(0.087)}{0.69}$ & $\underset{(0.096)}{0.69}$ & $\underset{(0.012)}{0.66}$ & $\underset{(0.066)}{0.64}$\\ \hline
    \begin{tabular}{@{}c@{}}Multi-Res \\ Attention\end{tabular} & $\underset{(0.0068)}{\textbf{0.85}}$ & $\underset{(0.025)}{\textbf{0.90}}$ & $\underset{(0.022)}{\textbf{0.91}}$ & $\underset{(0.013)}{\textbf{0.70}}$\\ \hline
\end{tabular} 
    \label{tab:result}
\end{table}

\subsection{Discussion}
Table \ref{tab:result} reports the average accuracy over 5 iterations for the balanced data sets in table \ref{tableDataSetSummary}. As expected, \emph{OnlyStrong} performs the worst since it is limited to the small labeled data. Semi-supervised learning baseline \emph{SSRManifold} shows improvement over \emph{OnlyStrong}, since it makes use of the features on the unlabeled data, but it does not use the label and hence falls short of the other methods. \emph{WeaSL} optimizes for fine-resolution level accuracy through CCN modeling of the coarse-resolution labels as group-label for fine-resolution instances. Thus, it benefits from using the coarse-resolution labeled data in conjunction with the fine-resolution labeled data. \emph{Augment} is another way to use the coarse-resolution data along with the fine-resolution data and therefore shows an increase in performance from \emph{OnlyStrong}, but it uses a weak MIL notion for the agreement between the coarse-resolution and fine-resolution labels.

\begin{figure}[!htb]
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{IMAGES/Attention_Weights_NLP.pdf}
        \label{fig:NLP}
    \end{subfigure}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth]{IMAGES/Attention_Weights.pdf}
        \label{fig:House1}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth]{IMAGES/Att_Weight_1.png}
        \label{fig:House2}
    \end{minipage}
    \caption{Visualization of Attention Weights}
    \label{fig:Att_Weights Examples}
\end{figure}



==> introduction.tex <==
\section{Introduction}
%Here comes the sun!

% Classifying spatio-temporal phenomena at multiple resolutions using multiview regularization and attention mechanism

%% The prevalence of spatio-temporal data
Many real world phenomena in a number of domains including earth science, epidemiology, brain imaging, criminology etc are inherently spatio-temporal in nature. Spatio-temporal data is most commonly collected as raster data \cite{AtluriSurvey} where the underlying spatio-temporal field is observed at fixed locations in space and fixed points in time. Examples of spatio-temporal raster data sets include brain activity measurements through fMRI video sequences,  time series of air quality measurements through ground sensors at a weather station, raster images of reflectance data collected by satellites orbiting the Earth. 

A key characteristic of raster data sets is the resolution at which the data is collected. The same spatio-temporal field might be observed at different resolutions in space and time across different data sets. Data sets collected at different resolutions might differ in terms of the kind of features that they have and the availability of training samples at that resolution. However, since they all observe the same underlying spatio-temporal field, inferences made using data observed at different resolutions have to be consistent and thus, they can complement each other.


As an example, table ~\ref{tab:data-sets} shows the spatial and temporal resolutions for few of the publicly available raster data sets in the remote sensing domain. These data sets are used for various environmental applications, prominently among which is the task of mapping land cover and land use across the globe over time \cite{AnujMagazine}. From the table, one can clearly see that there is a wide range of available resolutions. While we may want high resolution maps of land use, using coarser resolution data sets in conjunction can be very advantageous. Coarser spatial resolution satellite products such as MODIS (500m*500m pixels) are observed more frequently in time (every 8 days), while very fine resolution products such as x (10cm*10cm pixels) might only be available for select dates. Coarser spatial resolution products have been collected for several decades, unlike some of the fine resolution products, so historical analyses are not possible with fine resolution data sets. Moreover, it might be easier to procure training data at coarser resolutions since there are many good quality land cover products that already exist at this resolution. Finally, since every satellite product typically observes the Earth across different ranges of wavelengths, the features for the same location across different satellite products are different and hence complementary.

In this paper, we consider the problem of predicting a class of interest on a spatio-temporal field using raster data sets at multiple resolutions. Generally, one operates in a setting where we are trying to predict the class of interest at a single resolution, with features and training samples provided for that resolution. In contrast, in our setting, training data is available for a limited number of instances at each resolution, that informs us of the presence or absence of the class of interest, when observed from that resolution. The different resolutions can be seen as different \emph{views} that describe the same data set, on which a predictive model is being learned. The theory of multi-view learning, which considers predictive modeling settings with multiple \emph{views} of the data, states that under the assumption that the feature spaces corresponding to the two views are independent of each other, it is possible for models trained separately on each \emph{view} of the data to learn from the others. Therefore, in our case, instead of separately learning models to predict the phenomenon at different resolutions, we propose to simultaneously learn these models while maintaining the consistency of predictions between resolutions on the entire data set, labeled or unlabeled. This has the following advantages (1) Utilizes an independent feature space (2) Utilizes unlabeled data and (3) Mitigates lack of labeled data from either resolution. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{IMAGES/Resolution.png}
    \caption{This figure shows a small region in Juba, South Sudan and the corresponding labels (urban land) as observed from 30 m resolution and 10 m resolution. Note how only part of the region seems urban from the finer resolution although all of it is urban at the coarse resolution. Moreover, the fraction of urban fine resolution instances within a urban coarse resolution instance can have a large variability.}
    \label{fig:resolution}
\end{figure}

However, the key challenge in applying the multi-view learning approach in our case is the many-to-one nature of correspondence between instances from one view to the other. Figure ~\ref{fig:resolution} shows a caricature demonstrating this challenge in enforcing the consistency idea. The example considers the problem of predicting urban areas using two raster data sets with different spatial resolutions. Note that the number of fine resolution instances classified as urban within an urban coarse resolution instance is variable within the data set. In this paper, we propose two strategies to handle this many-to-one correspondence between a pair of resolutions, coarse and fine - (1) Using a multi-instance approach, where the presence of even a single instance of the class of interest among the finer resolution instances makes the corresponding coarse resolution instance positive. (2) Using the features of the coarse resolution instance and the corresponding fine resolution instances to compute the matching instances through an attention mechanism.

\begin{table*}[t]
    \centering
    \caption{The variability in the available raster data sets for the remote sensing domain}
    \begin{tabular}{|c|c|c|c|}
    \hline 
    DATASET & TEMPORAL RESOLUTION & SPATIAL RESOLUTION & AVAILABILITY\\\hline
    MODIS/VIIRS & 8 days & 250 metres & via NASA\\\hline
    LANDSAT & 16 days & 30 metres & via USGS\\\hline
    SENTINEL & 10 days & 10 metres & via ESA\\\hline
    PLANETSCOPE & daily & 3 metres & commercially available\\\hline
    \end{tabular}
    \label{tab:data-sets}
\end{table*}

\subsection{Contributions}
In a nutshell, we make the following contributions in this work
\setlist{nolistsep}
\begin{enumerate}
    \item Formalize the problem of classifying phenomena across multiple resolutions in a multi-view framework.
    \item Propose multiple strategies to implement the multi-view framework that handle the many-to-one correspondence across resolutions.
    \item Demonstrate the utility of the proposed method on land cover mapping problems of great environmental significance. 
\end{enumerate}

==> method.tex <==
\section{Method} \label{methodsSection}
\subsection{Problem setting}
We consider a two-class image segmentation problem where the goal is to learn two models at different resolutions that predicts the binary class $y \in \{0,1 \}$ for a test instance given its features $\bm{x_f}$ and $\bm{x_c}$ at both fine and coarse resolutions. During the training phase we have two sets of features for the same instance:
\setlist{nolistsep}
\begin{itemize}
    \item[a.] Coarse-resolution data set of $N_c$ instances $\{ (\bm{x_i}, y_i) \}_{i=1}^{N_f}$ having features $\bm{x_i}$ and labels $y_i$ for each instance $i$.
    \item[b.] Fine-resolution data set of $N_f$ instances $\{ (\bm{x_i}, y_i) \}_{i=1}^{N_f}$ having features $\bm{x_i}$ and labels $y_i$ for each instance $i$.
\end{itemize}
Being higher resolution, $N_f>N_c$ as both are the images of the same region.

\subsection{Proposed model}
We now present a Multi-Resolution Learning algorithm to improve the performance of the classifiers trained on either of the available data-sets i.e. coarse and fine resolution. We achieve this increase in performance by regularizing with consistency loss that ensures the consistency in predictions between the models of different resolution.
We consider a function $f(\bm{x})$ that models $Pr(y =1 | \bm{x})$ as the classifier. The generated probability can be thresholded at 0.5 to convert it to a binary prediction. We learn one such classifier at the coarse resolution data-set i.e.,
\begin{equation}
    \hat{y_c} = P(y=1|x_c,w_c) = \frac{1}{1+e^{-f(x_c, w_c)}}
\end{equation}
where, $w_c$ are the parameter to the model at coarse resolution, $x_c$ and $y_c$ are the coarse resolution input and output respectively.
Similarly another classifier is learned at the fine-resolution data-set,
\begin{equation}
    \hat{y_f} = P(y=1|x_f,w_f) = \frac{1}{1+e^{-f(x_f, w_f)}}
\end{equation}
where, $w_f$ are the parameter to the model at fine-resolution, $x_f$ and $y_f$ are the fine-resolution input and output respectively.

\subsection{Training Objective}
Our objective function is a sum of the performances over the two kinds of training instances - coarse ($O_c$) and fine ($O_f$) as well another function which measures the consistency in predictions by these two models when the data obtained from these two different sources belong to the same region.
The optimal parameters $\hat{w_c}$ and $\hat{w_f}$are estimated as,
\begin{equation} \label{total}
\hat{w_c}, \hat{w_f} = \argmax_{w_c, w_f} O_c + \lambda O_f + \delta O_x
\end{equation}
where $\lambda$ and $\delta$ are the weighting parameter fixed using cross-validation.

\subsubsection{Performance on coarse-resolution and fine-resolution instances}
The performance of model $f_c$ with parameters $w_c$ over the coarse-resolution samples $O_c(w_c)$ is simply the cross-entropy loss between the predicted probability $\hat{y_c}$ and the true labels $y_c$, which can be computed as,
\begin{equation} \label{eq_coarse}
    O_c(w_c) = \frac{1}{N_c}\sum_{i=1}^{N_c}  y^i_c log(\hat{y^i_c}) + (1-y^i_c)log(1-\hat{y^i_c})
\end{equation}
Similarly, the performance of model $f_f$ with parameters $w_f$ over the coarse-resolution samples $O_f(w_f)$ is the cross-entropy loss between the predicted probability $\hat{y_f}$ and the true labels $y_f$ computed as,
\begin{equation} \label{eq_fine}
    O_f(w_f) = \frac{1}{N_f}\sum_{i=1}^{N_c}  y^i_c log(\hat{y^i_c}) + (1-y^i_c)log(1-\hat{y^i_c})
\end{equation}
Note that both coarse resolution and fine resolution labels may not be available for the same region, thus these performances are on independent regions wherever those respective labels are available.

\subsubsection{Consistency measure of the models over a region}
Both the models are applied to the same region in the training phase and the predictions are recorded. This measure does not require the labels to be available and thus can be applied to any region irrespective of the availability of both coarse and fine resolution labels. Depending on the resolution difference of the datasets, for every coarse-resolution pixel of a region we have a fixed number (K) of fine-resolution pixels. For e.g. every coarse-resolution pixel will have corresponding 9 fine-resolution pixels if the coarse-resolution and fine-resolution data-set has 30m and 10m spatial resolution respectively as illustrated in figure[].

For consistency measure, we consider $N^x_c$ such coarse-resolution pixels and their corresponding $KN^x_f$ fine-resolution pixels. The consistency measure modelled as Multi-Instance Learning is compurted as,
\begin{equation} \label{eq_cons}
    O_x(w_c, w_f) = \frac{1}{N^x_c}\sum_{i=1}^{N^x_c}  (y^i_c -  \max_{j \in K} y^j_f)^2
\end{equation}
To keep the objective function differentiable, the maximum over different values of the fine-resolution predictions $y^j_f$ is computed using a softmax function i.e the different $y^j_f$'s are converted to a softmax distribution and the final value is the weighted sum of the fine-resolution predictions $y^j_f$ with the corresponding weight from the softmax distribution\footnote{Higher values of base other than $e$ can be used for softmax to make the function sharper}. i.e,
\begin{equation}
    O_x(w_c, w_f) = \frac{1}{N^x_c}\sum_{i=1}^{N^x_c}  (y^i_c -  \frac{\sum_{j \in K}y^j_f e^{y^j_f}}{\sum_{j \in K} e^{y^j_f}})^2
\end{equation}

\subsubsection{Final Objective Function}
As shown in eq.\eqref{total} the final objective function is the weighted sum of eq.\eqref{eq_coarse}, eq.\eqref{eq_fine} and eq.\eqref{eq_cons}. Figure[] shows a linear form of function $f$, however one could add more hidden layers for a non-linear model such as deep neural networks.

==> method_v1.tex <==
% edits by Guru
\section{Method}

% Problem setting

% Multi-view framework - add background on multi-view learning

% Multi-instance solution - add background on multi-instance learning

% Attention mechanism solution - add background on attention mechanism

\subsection{Problem Setting}
In this paper, we consider the problem of classifying a spatio-temporal field on multiple resolutions. Data instances at every resolution $1 \leq k \leq NR$ can be described through attributes $(\bm{x}, l, y)$ described as follows
\setlist{nolistsep}
\begin{enumerate}
    \item Features $\bm{x} \in R^{D_k}$, where ${D_k}$ is the dimensionality of the features observed in the $k$th resolution
    \item Location $l$ that describes the voxel id of the observation that encodes the location in space and the point in time where each instance is observed.
    \item Label $y \in \{0,1\}$ that encodes the presence ($y=1$) or absence ($y =0$) of the class of interest at location $l$
\end{enumerate}
\textbf{Goal: }To learn classification models $\bm{w}_k$ at every resolution $k$ that can take the features $\bm{x^k}$ observed for an instance on that resolution and predict its corresponding label $y^k$. \\ \hfill
\textbf{Training data: }During the training phase, for each resolution $k$, we are provided a set $T_l^k$ of $N_l^k>0$ labeled samples $\{ \bm{x}^k_i, l^k_i, y^k_i\}_{i=1}^{N_l^k}$. In addition, we have unlabeled data for a large region $RU$ of the spatio-temporal field at every resolution i.e we have features $\bm{x}^k_i$ for every observable location $l$ within the region $RU$ at resolution $k$, forming a unlabeled training data set $T_u^k$ of $N_u^k$ samples $\{ \bm{x}^k_i, l^k_i\}_{i=1}^{N_u^k}$.



\subsection{Multi-view framework}
Classification models $\bm{w}_k$ are learned at every resolution $k \in \{1 \cdots, NR\}$. In particular, classifier $f_{k}(\bm{x^{k}}; \bm{w}_{k})$ at resolution $k$ with parameters $\bm{w}_k$ models $Pr(y^k =1 | \bm{x}^k)$, where $y^k$ is the label at that resolution. We place no restriction on the actual form of $f$. It could take any form like LSTMs for temporal data or CNNs for spatial data or more traditional classifiers like a neural network with one hidden layer. However, instead of learning the classifiers at different resolutions independently, as would be the case in a conventional approach, we propose to use the large number of unlabeled data available on the same region $RU$ of the spatio-temporal field to enforce consistency in predictions across resolutions and thus, make the models on different resolutions learn from each other. Thus, the objective function takes the following form,

\begin{equation}
    \label{eqObjFun}
    \begin{split}
        O(\bm{w_1}, &\cdots, \bm{w_{NR}}) = \sum_{k=1}^{NR} L(T_l^k; \bm{w_k}) + \\ &\sum_{k_1=1}^{NR-1} \lambda_{k_1} \sum_{k_2=k_1 + 1}^{NR} D(pred(T_u^{k_1}; \bm{w}_{k_1}), pred(T_u^{k_2}; \bm{w}_{k_2}))
    \end{split}
\end{equation}

The first term in the objective function is the loss over labeled samples while the second term is a regularization term that enforces the consistency of predictions across resolutions on the unlabeled instances i.e $L(T_l^k; \bm{w_k})$ is the loss over the labeled training instances $T_l^k$ on the $k$th resolution and the function $D()$ captures the consistency of the predictions between every pair of resolutions. 

\subsubsection{Defining consistency across resolutions}
The choice of function $L()$ in equation \ref{eqObjFun} is standard. Defining the consistency function $D()$ is non-trivial because of the lack of an one-to-one mapping between instances across a pair of resolutions, as would be the case in traditional multi-view problems. Given a pair of resolutions - coarse and fine, one can define a many-to-one mapping of instances from the fine resolution to the coarse resolution by using a nearest neighbor approach. i.e every fine resolution instance is assigned to the coarse resolution instance with the closest location to it. Subsequently, the consistency of predictions on the unlabeled instances between a pair of resolutions boils down to defining the consistency between every coarse resolution instance and its corresponding fine resolution instances. In particular, the consistency term in equation \ref{eqObjFun} can be rewritten as, 

\begin{equation*}
%\label{eqFuncd}
\begin{split}
    D(&pred(T_u^{k_1}; \bm{w}_{k_1}), pred(T_u^{k_2}; \bm{w}_{k_2})) = \\
    &\sum_{i \in T_u^{k_1}}  d(\bm{x_i^{k_1}}, \{\bm{x_j^{k_2}} | j \in S_i \text{ and } j \in T_u^{k_2} \}, \bm{w_{k_1}}, \bm{w_{k_2}})
\end{split}
\end{equation*}
where the summation is over all unlabeled instances $i$ in the coarser resolution $k_1$. Also, the set $S_i$ denotes the unlabeled instances in fine resolution $k_2$ that are closest in location to instance $i$ from the coarser resolution. Thus, the objective function can be rewritten as,
\begin{equation}
    \label{eqObjFun2}
    \begin{split}
        &O(\bm{w_1}, \cdots, \bm{w_{NR}}) = \sum_{k=1}^{NR} L(T_l^k; \bm{w_k}) + \\ &\hspace{-2mm}\sum_{k_1=1}^{NR-1} \hspace{-1mm}\lambda_{k_1} \hspace{-3mm} \sum_{k_2=k_1 + 1}^{NR} \sum_{i \in T_u^{k_1}}  d(\bm{x_i^{k_1}}, \{\bm{x_j^{k_2}} | j \in S_i \& j \in T_u^{k_2} \}, \bm{w_{k_1}}, \bm{w_{k_2}})
    \end{split}
\end{equation}



In this work, we propose two strategies to define the consistency of predictions $d()$ between a coarse resolution instance and its corresponding fine resolution instances - (1) Multi-instance learning (2) Attention mechanism

\subsection{Multiple Instance Learning (MIL) solution}
Multiple Instance Learning (MIL) \cite{MILSurvey1, MILSurvey2} considers the problem of learning predictive models to label groups of instances, in contrast to traditional settings where the goal is to label individual instances. Typical MIL classification settings operate under the presence-based assumption\cite{MILSurvey1} which states that a group has a positive label when at least one of its constituting instances has a positive label and it has a negative label when all of its constituting instances have a negative label as well. Figure \ref{fig:MILsetting} shows a caricature for the MIL assumption. MIL forms an direct way to define function $d()$ in equation \ref{eqObjFun2} that models the many-to-one relationship between an instance of a coarse resolution and its corresponding instances in the finer resolution. Given an instance $i$ from a coarse resolution $k_1$ and its corresponding instances $S_i$ from a fine resolution $k_2$, the prediction for the coarse resolution label can be written in two ways - first using the model on resolution $k_1$

\begin{equation*}
    Pr(y_i^{k_1} | \bm{x_{i}^{k_1}}) = f_{k_1}(\bm{x_{i}^{k_1}}; \bm{w}_{k_1})
\end{equation*}
Secondly, the label at $k_1$ can also be predicted using corresponding instances on $k_2$ using the MIL assumption.
\begin{equation*}
    Pr(y_i^{k_1} | \{\bm{x_{j}^{k_2}} | j \in S_i\} ) = \max_{j \in S_i} f_{k_2}(\bm{x_{j}^{k_2}}; \bm{w}_{k_2})
\end{equation*}

Note that taking the maximum of the probabilities for  instance-level for constituting instances is one way to implement the presence-based MIL assumption\cite{MILR}. Thus, the function $d()$ in equation \ref{eqObjFun2} can be defined as,
\begin{equation*}
\begin{split}
    d(\bm{x_i^{k_1}}, &\{\bm{x_j^{k_2}} | j \in S_i \text{ and } j \in T_u^{k_2} \}, \bm{w_{k_1}}, \bm{w_{k_2}}) = \\
    &\displaystyle\left(f_{k_1}(\bm{x_{i}^{k_1}}; \bm{w}_{k_1}) - \max_{j \in S_i} f_{k_2}(\bm{x_{j}^{k_2}}; \bm{w}_{k_2})\displaystyle\right)^2
\end{split}
\end{equation*}
Since we use gradient descent algorithm to learn the optimal parameters for our models, we want our objective functions to be differentiable and hence, in our implementation, the max function is replaced by its differentiable softmax approximation.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{IMAGES/standardMIL.pdf}
    \caption{Presence-based assumption in Multiple Instance Learning (MIL) settings. If a group has a positive label, at least one instance within it is positive. Conversely, a negative group is made of all negative instances.}
    \label{fig:MILsetting}
\end{figure}

\subsection{Attention mechanism solution}
While the multiple-instance learning approach is a logical way to model the many-to-one relationship between instances of different resolutions, it might be a sub-optimal way to share information through this many-to-one correspondence. There could be a large variation in the number of positive fine resolution instances within a coarse resolution instance. Thus, by defining correspondence based on just one instance (with the maximum probability) or even a fixed fraction of instances does not capture the exact relationship between the two resolutions. Instead, we propose to parametrize the learning of this relationship so that we adaptively learn the most relevant instances on the finer resolution to predict the label on the coarser resolution. Recently, attention models \cite{AttentionNLP} have been proposed for Natural Language Processing (NLP) tasks that utilize features to assign relevance of instances to one another with respect to a certain prediction task. In our problem, we propose to use the concept of attention to assign relevance to fine resolution instances in the context of predicting the label on the corresponding coarser resolution instance. In particular, given a coarse resolution instance $i$ at resolution $k_1$ and corresponding fine resolution instances $S_i$ on resolution $k_2$, the attention weight $a_j$ for every instance $j \in S_i$ is defined as,
\begin{equation*}
    a_j^{k_2} = \frac{g([\bm{h_j^{k_2}}, \bm{h_i^{k_1}}]; \bm{w}_a)}{\sum_{k \in S_i}{g([\bm{h_k}, \bm{h_i}]; \bm{w}_{a{k_1}{k_2}})}}
\end{equation*}
where $h_j^{k_2}$ and $h_i^{k_1}$ are hidden representations for the instances obtained from models $f^{k_2}$ and $f^{k_1}$ respectively. For simpler models these could just be $\bm{x}_j^{k_2}$ and $\bm{x}_i^{k_1}$. Also, square brackets such as $[\bm{h_j^{k_2}}, \bm{h_i^{k_1}}]$ denotes vector concatenation of the elements within. Given these attention weights, a representation for all instances in $S_i$ can be computed as $\sum_{j \in S_i} a_j^{k_2} h_j^{k_2}$. This aggregated representative hidden state can then be fed into model $f^{k_2}$ to obtain the prediction for $Pr(y_i^{k_1} | \{\bm{x_{j}^{k_2}} | j \in S_i\} )$. The definition for consistency function $d()$ in equation \ref{eqObjFun2} is the similar as in the MIL case i.e 
\begin{equation*}
\begin{split}
    d(\bm{x_i^{k_1}}, &\{\bm{x_j^{k_2}} | j \in S_i \text{ and } j \in T_u^{k_2} \}, \bm{w_{k_1}}, \bm{w_{k_2}}, \bm{w}_{a{k_1}{k_2}}) \\
    =&\displaystyle\left(Pr(y_i^{k_1} | \bm{x_{i}^{k_1}}) - Pr(y_i^{k_1} | \{\bm{x_{j}^{k_2}} | j \in S_i\} )\displaystyle\right)^2 \\
    =& \displaystyle\left(f_{k_1}(\bm{x_{i}^{k_1}}; \bm{w}_{k_1}) - Pr(y_i^{k_1} | \sum_{j \in S_i} a_j^{k_2} h_j^{k_2} )\displaystyle\right)^2 \\
    =& \displaystyle\left(f_{k_1}(\bm{x_{i}^{k_1}}; \bm{w}_{k_1}) - f_{k_2}^{'}(\sum_{j \in S_i} a_j^{k_2} h_j^{k_2}; \bm{w}_{k_2})\displaystyle\right)^2
\end{split}
\end{equation*}
where $f_{k_2}^{'}$ is the part of the model $f^{k_2}$ that generates the predictions $y^{k_2}$ once the hidden states $h^{k_2}$ are computed. Figure \ref{fig:attentionMethods} shows a sketch of the proposed attention based model and the computation of the corresponding objective function.


\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{IMAGES/Attention.png}
    \caption{Attention mechanism based solution to the multi-resolution classification problem. Rather than assuming that a fixed number of instances at the finer resolution contribute to the label at the coarse resolution, this model adaptively predicts instances at the finer resolution that are best suited to predict this particular coarse resolution instance.}
    \label{fig:attentionMethods}
\end{figure*}

==> titleAuthorList.tex <==
%\title{Classifying multi-resolution data using multi-view regularization and attention mechanism}

% alternate title
%\title{Classifying spatio-temporal phenomena at multiple resolutions using multi-view regularization and attention mechanism}
\title{Multi-view Semi-supervised Classification using Attention-based Regularization on Coarse-resolution Data}

\author{
Guruprasad Nayak$^1$\footnote{These authors contributed equally to this article} \and 
Rahul Ghosh$^1$*\and
Xiaowei Jia$^1$\and
Varun Mithal$^2$\and
Vipin Kumar$^1$
}
\date{$^1$University of Minnesota, \{nayak013, ghosh128, jiaxx221, kumar001\}@umn.edu
\\$^2$LinkedIn, varunmithal@gmail.com}
\maketitle
